Distinguished In Uniform: Self Attention Vs. Virtual Nodes

Graph Transformers (GTs) such as SAN and GPS are graph processing models that combine Message-Passing GNNs (MPGNNs) with global Self-Attention. They were shown to be universal function approximators, with two reservations: 1. The initial node features must be augmented with certain positional encodings. 2. The approximation is non-uniform: Graphs of different sizes may require a different approximating network. We first clarify that this form of universality is not unique to GTs: Using the same positional encodings, also pure MPGNNs and even 2-layer MLPs are non-uniform universal approximators. We then consider uniform expressivity: The target function is to be approximated by a single network for graphs of all sizes. There, we compare GTs to the more efficient MPGNN + Virtual Node architecture. The essential difference between the two model definitions is in their global computation method -- Self-Attention Vs Virtual Node. We prove that none of the models is a uniform-universal approximator, before proving our main result: Neither model's uniform expressivity subsumes the other's. We demonstrate the theory with experiments on synthetic data. We further augment our study with real-world datasets, observing mixed results which indicate no clear ranking in practice as well.

==> Tables/LRGB-Full.tex <==
\begin{table*}[t]
\caption{
    Performance of our models on the Long-Range Graph Benchmark.
}
\label{lrgb_results_full}
\begin{center}
\begin{small}
\resizebox{\textwidth}{!}{
\textsc{
\begin{tabular}{lccccccc}
\toprule
Method      & PASCALVOC-SP & COCO-SP & PEPTIDES-FUNC & PEPTIDES-STRUCT & \multicolumn{3}{c}{PCQM-CONTACT} \\
            & Test F1 $\uparrow$ & Test F1 $\uparrow$ & Test AP $\uparrow$ & Test MAE $\downarrow$ & \multicolumn{3}{c}{Test MRR $\uparrow$} \\
            & & & & & raw & filter & ext. filter \\
\midrule
GCN         & 0.2078 ± 0.0031 & 0.1338 ± 0.0007 & 0.6860 ± 0.0050 & 0.2460 ± 0.0007 & 0.3424 ± 0.0007 & 0.3631 ± 0.0006 & 0.4526 ± 0.0006 \\
GINE        & 0.2718 ± 0.0054 & 0.2125 ± 0.0009 & 0.6621 ± 0.0067 & 0.2473 ± 0.0017 & 0.3509 ± 0.0006 & 0.3725 ± 0.0006 & 0.4617 ± 0.0005 \\
GatedGCN    & 0.3880 ± 0.0040 & 0.2922 ± 0.0018 & 0.6765 ± 0.0047 & 0.2477 ± 0.0009 & 0.3495 ± 0.0010 & 0.3714 ± 0.0010 & 0.4670 ± 0.0004 \\
GPS         & 0.4440 ± 0.0065 & 0.3884 ± 0.0055 & 0.6534 ± 0.0091 & 0.2509 ± 0.0014 & 0.3498 ± 0.0005 & 0.3722 ± 0.0005 & 0.4703 ± 0.0014 \\
\bottomrule
\end{tabular}
}
}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
%}


==> Tables/LRGB-VN.tex <==
\begin{table*}[t]
\caption{
    Performance measurements of VN-equipped models on the Long-Range Graph Benchmark.
    \first{First}, \second{second}, and \third{third} best values are marked in color.
    Methods marked with $^*$ did not use feature normalization on the computer vision datasets.
}
\label{tab:lrgb_results_vn}
\begin{center}
\begin{small}
\resizebox{\textwidth}{!}{
\textsc{
\begin{tabular}{llcccc}
\toprule
&Method      & PASCALVOC-SP & COCO-SP & PEPTIDES-FUNC & PEPTIDES-STRUCT \\
            & & Test F1 $\uparrow$ & Test F1 $\uparrow$ & Test AP $\uparrow$ & Test MAE $\downarrow$ \\
\midrule
\multirow{6}{*}{\rotatebox{90}{MPGNN \& Co}}
&\hyperlink{cite.tonshoff2023reassessingLRGB}{GCN}         & 0.2078 ± 0.0031 & 0.1338 ± 0.0007 & {0.6860 ± 0.0050} & \third{0.2460 ± 0.0007} \\
&\hyperlink{cite.tonshoff2023reassessingLRGB}{GINE}        & 0.2718 ± 0.0054 & 0.2125 ± 0.0009 & 0.6621 ± 0.0067 & {0.2473 ± 0.0017} \\
&\hyperlink{cite.tonshoff2023reassessingLRGB}{GatedGCN}    & 0.3880 ± 0.0040 & 0.2922 ± 0.0018 & 0.6765 ± 0.0047 & 0.2477 ± 0.0009 \\
&\hyperlink{cite.cai2023connection}{MPNN+VN ($>500\!\operatorname{k}$)} & 0.3103 ± 0.0068 & - & 0.6685 ± 0.0062 & 0.2488 ± 0.0021 \\
&\hyperlink{cite.gutteridge2023drew}{DRew}                 & 0.3314 ± 0.0024 & - & \first{0.7150 ± 0.0044} & 0.2536 ± 0.0015 \\
&\hyperlink{cite.toenshoff2023walking}{CRaWl} & \first{0.4588 ± 0.0079} & - & \second{0.7074 ± 0.0032} & 0.2506 ± 0.0022\\
\midrule
\multirow{5}{*}{\rotatebox{90}{Transformer}}
&\hyperlink{cite.kreuzer2021rethinking}{SAN}               & 0.3230 ± 0.0039 & 0.2592 ± 0.0158 & 0.6439 ± 0.0075 & 0.2545 ± 0.0012 \\
&\hyperlink{cite.rampavsek2022recipe}{GPS}                 & \second{0.4440 ± 0.0065} & \first{0.3884 ± 0.0055} & 0.6534 ± 0.0091 & 0.2509 ± 0.0014 \\
&\hyperlink{cite.he2023generalization}{Graph-ViT} ($>500\!\operatorname{k}$)          & - & - & 0.6876 ± 0.0059 & \first{0.2449 ± 0.0016} \\
&\hyperlink{cite.shirzad2023exphormer}{Exphormer}          & 0.3975 ± 0.0037 & \second{0.3455 ± 0.0009} & 0.6527 ± 0.0043 & 0.2481 ± 0.0007\\
&\hyperlink{cite.ma2023graph}{GRIT} & - & - & \third{0.6988 ± 0.0082} & \third{0.2460 ± 0.0012} \\
&\hyperlink{cite.ngo2023multiresolution}{MGT + WavePE} & - & - & 0.6817 ± 0.0064 & \second{0.2453 ± 0.0025}\\
\midrule
\multirow{2}{*}{\rotatebox{90}{VN}}
&GCN-VN      & 0.2950 ± 0.0058 &  0.2072 ± 0.0043  & 0.6779 ± 0.0043 & {0.2477 ± 0.0026} \\
&GatedGCN-VN & \third{0.4477 ± 0.0137} & \third{0.3244 ± 0.0025} & 0.6823 ± 0.0069 & {0.2475 ± 0.0018} \\
\bottomrule
\end{tabular}
}
}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
%}


==> Tables/LRGB.tex <==
% \begin{table*}[t]
% \caption{
%     Performance on the Long-Range Graph Benchmark. Baseline results are reported by \cite{dwivedi2022long}
% }
% \label{lrgb_results}
% \begin{center}
% \begin{small}
% \resizebox{\textwidth}{!}{
% \textsc{
% \begin{tabular}{lcccccc}
% \toprule
% Method     & \multicolumn{2}{c}{PASCALVOC-SP} & COCO-SP & PEPTIDES-FUNC & PEPTIDES-STRUCT & PCQM-CONTACT \\
%            & \multicolumn{2}{c}{Test F1 $\uparrow$} & Test F1 $\uparrow$ & Test AP $\uparrow$ & Test MAE $\downarrow$ & Test MRR $\uparrow$ \\
%            & Unnormalized & Normalized & & & & \\
% \midrule
% \hyperlink{cite.kipf2017semi}{GCN}                      & 0.1268 ± 0.0060 & - & 0.0841 ± 0.0010 & 0.5930 ± 0.0023 & 0.3496 ± 0.0013 & 0.3234 ± 0.0006 \\
% \hyperlink{cite.Keyulu18}{GINE}                         & 0.1265 ± 0.0076 & 0.2385 ± 0.0023 & 0.1339 ± 0.0044 & 0.5498 ± 0.0079 & 0.3547 ± 0.0045 & 0.3180 ± 0.0027 \\
% \hyperlink{cite.bresson2017residual}{GatedGCN}          & 0.2873 ± 0.0219 & 0.2938 ± 0.0023 & 0.2641 ± 0.0045 & 0.6069 ± 0.0035 & 0.3357 ± 0.0006 & 0.3242 ± 0.0008 \\
% \hyperlink{cite.dwivedi2020generalization}{Transformer} & 0.2694 ± 0.0098 & - & 0.2618 ± 0.0031 & 0.6326 ± 0.0126 & 0.2529 ± 0.0016 & 0.3174 ± 0.0020 \\
% \hyperlink{cite.kreuzer2021rethinking}{SAN}              & 0.3230 ± 0.0039 & - & 0.2592 ± 0.0158\clap{\,~$^\star$} & 0.6439 ± 0.0075 & 0.2545 ± 0.0012 & 0.3350 ± 0.0003 \\
% GPS              & 0.3748 ± 0.0109 & 0.4170 ± 0.0118 & 0.3412 ± 0.0044 & 0.6535 ± 0.0041 & 0.2500 ± 0.0005 & 0.3337 ± 0.0006 \\
% %\midrule
% %\textsc{CRaWl}                                               & \textbf{0.4588 ± 0.0079} & & \textbf{0.7074 ± 0.0032} & \textbf{0.2506 ± 0.0022} & \\
% \midrule
% GINE & - & 0.3640 ± 0.0069 & &  0.6749 ± 0.0099 & 0.2493 ± 0.0013 & 0.3329 ± 0.0014\\
% GINE+VN & - & 0.3710 ± 0.0092 & & 0.6705 ± 0.0047 & 0.2504 ± 0.0014 & \\
% GatedGCN & - & \textbf{0.4205} ± \textbf{0.0055} & & 0.6756 ± 0.0045 & 0.2524 ± 0.0018 & 0.3411 ± 0.0007\\
% GatedGCN+VN & - & \textbf{0.4446} ± \textbf{0.0103} & \textbf{0.3459} ± \textbf{0.0039} & \textbf{0.6836} ± \textbf{0.0083} & \textbf{0.2488} ± \textbf{0.0015} & \textbf{0.3490} ± \textbf{0.0007} \\
% \midrule
% GINE a) & - & 0.2742 ± 0.0045 & &  0.6832 ± 0.0048 & 0.2554 ± 0.0035 & \\
% GINE b) & - & 0.2834 ± 0.0028 & &  0.6627 ± 0.0068 & 0.2532 ± 0.0016 & \\
% GINE c) & - & 0.3640 ± 0.0069 & &  0.6749 ± 0.0099 & 0.2493 ± 0.0013 & \\
% GINE d) & - & 0.3710 ± 0.0092 & & 0.6705 ± 0.0047 & 0.2504 ± 0.0014 & \\
% \midrule
% GatedGCN a) & - & 0.3883 ± 0.0021 & & 0.6776 ± 0.0028 & 0.2559 ± 0.0002 & \\
% GatedGCN b) & - & 0.3733 ± 0.0016 & & 0.6471 ± 0.0043 & 0.2513 ± 0.0009 & \\
% GatedGCN c) & - & 0.4205 ± 0.0055 & & 0.6756 ± 0.0045 & 0.2524 ± 0.0018 & \\
% GatedGCN d) & - & \textbf{0.4446 ± 0.0103} & 0.3459 ± 0.0039 & 0.6836 ± 0.0083 & 0.2488 ± 0.0015 & 0.3490 ± 0.0007 \\
% GatedGCN e) & - & 0.4154 ± 0.0121 & & 0.6652 ± 0.0053 & & \\
% \bottomrule
% \end{tabular}
% }
% }
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}
% %}


% \begin{table*}[t]
% \caption{
%     Performance on the Long-Range Graph Benchmark. Baseline results are reported by \cite{dwivedi2022long}
% }
% \label{lrgb_results}
% \begin{center}
% \begin{small}
% \resizebox{\textwidth}{!}{
% \textsc{
% \begin{tabular}{lcccccc}
% \toprule
% Method     & \multicolumn{2}{c}{PASCALVOC-SP} & PEPTIDES-FUNC & PEPTIDES-STRUCT \\
%            & \multicolumn{2}{c}{Test F1} & Test AP & Test MAE \\
%            & Unnormalized & Normalized & &\\
% \midrule
% \hyperlink{cite.kipf2017semi}{GCN}                      & 0.1268 ± 0.0060 & - & 0.5930 ± 0.0023 & 0.3496 ± 0.0013 \\
% \hyperlink{cite.Keyulu18}{GINE}                         & 0.1265 ± 0.0076 & 0.1339 ± 0.0044 & 0.5498 ± 0.0079 & 0.3547 ± 0.0045  \\
% \hyperlink{cite.bresson2017residual}{GatedGCN}          & 0.2873 ± 0.0219 & 0.2641 ± 0.0045 & 0.6069 ± 0.0035 & 0.3357 ± 0.0006  \\
% \hyperlink{cite.dwivedi2020generalization}{Transformer} & 0.2694 ± 0.0098 & - & 0.6326 ± 0.0126 & 0.2529 ± 0.0016  \\
% \hyperlink{cite.kreuzer2021rethinking}{SAN}             & 0.3230 ± 0.0039 & - & 0.6439 ± 0.0075 & 0.2545 ± 0.0012 & \\
% GPS                                                     & 0.3748 ± 0.0109 & 0.4170 ± 0.0118 & 0.6535 ± 0.0041 & 0.2500 ± 0.0005 \\
% %\midrule
% %\textsc{CRaWl}                                               & \textbf{0.4588 ± 0.0079} & & \textbf{0.7074 ± 0.0032} & \textbf{0.2506 ± 0.0022} & \\
% \midrule
% GINE & - & 0.2834 ± 0.0028 & 0.6627 ± 0.0068 & 0.2532 ± 0.0016 & \\
% GatedGCN & - & 0.3733 ± 0.0016 & 0.6471 ± 0.0043 & 0.2513 ± 0.0009 & \\
% \bottomrule
% \end{tabular}
% }
% }
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}
% %}



% -------------------------------------------------------------- New Table -----------------------------------------------------------------------------------------


\begin{table*}[t]
\caption{
    Performance on the Long-Range Graph Benchmark. Baseline results are reported by \cite{dwivedi2022long}
}
\label{lrgb_results}
\begin{center}
\begin{small}
\resizebox{\textwidth}{!}{
\textsc{
\begin{tabular}{lccccc}
\toprule
Method     & PASCALVOC-SP & COCO-SP & PEPTIDES-FUNC & PEPTIDES-STRUCT & PCQM-CONTACT \\
           & Test F1 $\uparrow$ & Test F1 $\uparrow$ & Test AP $\uparrow$ & Test MAE $\downarrow$ & Test MRR $\uparrow$ \\
\midrule
\hyperlink{cite.kipf2017semi}{GCN}                      & 0.1268 ± 0.0060 & 0.0841 ± 0.0010 & 0.5930 ± 0.0023 & 0.3496 ± 0.0013 & 0.3234 ± 0.0006 \\
\hyperlink{cite.Keyulu18}{GINE}                         & 0.1265 ± 0.0076 & 0.1339 ± 0.0044 & 0.5498 ± 0.0079 & 0.3547 ± 0.0045 & 0.3180 ± 0.0027 \\
\hyperlink{cite.bresson2017residual}{GatedGCN}          & 0.2873 ± 0.0219 & 0.2641 ± 0.0045 & 0.6069 ± 0.0035 & 0.3357 ± 0.0006 & 0.3242 ± 0.0008 \\
\hyperlink{cite.dwivedi2020generalization}{Transformer} & 0.2694 ± 0.0098 & 0.2618 ± 0.0031 & 0.6326 ± 0.0126 & 0.2529 ± 0.0016 & 0.3174 ± 0.0020 \\
\hyperlink{cite.kreuzer2021rethinking}{SAN}             & 0.3230 ± 0.0039 & 0.2592 ± 0.0158\clap{\,~$^\star$} & 0.6439 ± 0.0075 & 0.2545 ± 0.0012 & 0.3350 ± 0.0003 \\
GPS                                                     & 0.3748 ± 0.0109 & 0.3412 ± 0.0044 & 0.6535 ± 0.0041 & 0.2500 ± 0.0005 & 0.3337 ± 0.0006 \\
%\midrule
%\textsc{CRaWl}                                               & \textbf{0.4588 ± 0.0079} & & \textbf{0.7074 ± 0.0032} & \textbf{0.2506 ± 0.0022} & \\
\midrule
GCN & 0.2069 ± 0.0031 & 0.1281 ± 0.0013 & 0.6860 ± 0.0050 & \textbf{0.2459 ± 0.0007}  & \\
GINE & 0.2728 ± 0.0074 & & 0.6621 ± 0.0067 & 0.2472 ± 0.0017 & \\
GatedGCN & 0.3931 ± 0.0010 & 0.2798 ± 0.0033 & 0.6765 ± 0.0047 & 0.2477 ± 0.0009 & 0.3535 ± 0.0018 \\
%\midrule
GPS & \textbf{0.4440 ± 0.0065} & 0.3945 ± 0.0052 & 0.6533 ± 0.0091 & 0.2509 ± 0.0014 & 0.3498 ± 0.0005 \\
MPNN+TL & 0.4241 ± 0.0030 & 0.3235 ± 0.0063 & \textbf{0.6914 ± 0.0064} & 0.2508 ± 0.0009 & \\
MPNN+TL+VN & \textbf{0.4451 ± 0.0061} & 0.3544 ± 0.0025 & 0.6852 ± 0.0008 & 0.2484 ± 0.0009 &\\
\bottomrule
\end{tabular}
}
}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
%}


==> Tables/OGB.tex <==
%\resizebox{\textwidth}{!}{
\begin{table*}[t]
\caption{
    Performance on benchmark datasets, \first{first}, \second{second}, and \third{third} best method are marked in color. $^\star$ means pretrained on external data.
}
%tabellen reformatieren für camera ready https://tex.stackexchange.com/questions/419825/column-alignment-for-si-error-range 
\label{zinc_results}
\label{tab:zincAndOgb}
\begin{center}
% \begin{tiny}
\textsc{
\resizebox{\textwidth}{!}{
\begin{tabular}{llccc}
\toprule
&Method     & ZINC & OGB-CODE2 & OGB-MOLPCBA \\
&           & Test MAE $\downarrow$ & Test F1 $\uparrow$ & Test AP $\uparrow$ \\
\midrule
\multirow{9}{*}{\begin{tikzpicture}\node[rotate=90] at (0,0){\small MPGNN/Others};\end{tikzpicture}}
&\hyperlink{cite.kipf2017semi}{GCN}                             & 0.367 ± 0.011 & 0.1507 ± 0.0018 & 0.2483 ± 0.0037 \\
&\hyperlink{cite.Keyulu18}{GIN}                                 & 0.526 ± 0.051 & 0.1495 ± 0.0023 & 0.2703 ± 0.0023 \\ % (VN,F) für Molpcba
&\hyperlink{cite.bresson2017residual}{GatedGCN}                 & 0.214 ± 0.006 & - & - \\
% &\hyperlink{cite.DBLP:journals/corr/HamiltonYL17}{GraphSage}    & 0.398 ± 0.002 & - & - \\
&\hyperlink{cite.velivckovic2017graph}{GAT}                     & 0.384 ± 0.007 & 0.1569 ± 0.0010 & - \\
% &\hyperlink{cite.maron2019provably}{3WLGNN}                     & 0.303 ± 0.068 & - & - \\
&\hyperlink{cite.corso2020principal}{PNA}                       & 0.142 ± 0.010 & 0.1570 ± 0.0032 & 0.2838 ± 0.0035 \\
% & \hyperlink{cite.brossard2020graph}{GINE+}                     & - & - & 0.2917 ± 0.0015\\
& \hyperlink{cite.gineappnp}{GINE+\&APPNP}                      &-& - & 0.2979 ± 0.0030\\
% &\hyperlink{cite.NEURIPS2021_8462a7c2}{Nested GIN}                 & - & - & 0.2832 ± 0.0041 \\
&\hyperlink{cite.zhao2022from}{GIN-AK+}                 & 0.080 ± 0.001 & - & 0.2930 ± 0.0044 \\
% &\hyperlink{cite.bouritsas2020improving}{GSN}                 & \clap{$^\star$~\,}0.108 ± 0.018 & - &-\\
% &\hyperlink{cite.CIN}{CIN}                 & 0.079 ± 0.006 & - & - \\
&\hyperlink{cite.toenshoff2023walking}{CRaWl}    & 0.085 ± 0.004 & - & 0.2986 ± 0.0025 \\
&\hyperlink{cite.yang2023towards}{PDF} & \second{0.066 ± 0.002} & - & 0.3031 ± 0.0026 \\
\midrule
\multirow{6}{*}{\begin{tikzpicture}\node[rotate=90] at (0,0){\small Transformer};\end{tikzpicture}}
& GPS & 0.070 ± 0.004 & \third{0.1894 ± 0.0024} & 0.2907 ± 0.0028\\
& \hyperlink{cite.lgi-gt}{LGI-GT} & 0.069 ± 0.002 & \first{0.1948 ± 0.0024} & 0.3040 ± 0.0029 \\
%&\hyperlink{cite.beaini2020directional}{DGN}                 & $^\dag$0.168 ± 0.003\phantom{$^\dag$} & ~~- & \textbf{72.840} ± \textbf{0.420} &- \\
%&\hyperlink{cite.fey2020hierarchical}{HIMP}                & $^\ast$0.151 ± 0.006\phantom{$^\ast$} & ~~- & ~~-  &-\\
&\hyperlink{cite.NEURIPS2021_b4fd1d2c}{SAN}                 & 0.139 ± 0.006 & - & 0.2765 ± 0.0042 \\
&\hyperlink{cite.chen2022structure}{SAT}                 & 0.094 ± 0.008 & \second{0.1937 ± 0.0028} & - \\
&\hyperlink{cite.ma2023graph}{GRIT} & \first{0.059 ± 0.002} & - & - \\
&\hyperlink{cite.ying2021transformers}{Graphormer} & 0.122 ± 0.006 & - & \second{\clap{$^\star$~~}0.3140 ± 0.0032} \\
% \midrule
\midrule
\multirow{2}{*}{\begin{tikzpicture}\node[rotate=90] at (0,0){\small Ours\!\!\!}; \end{tikzpicture}}
& MPGNN & \third{0.067 ± 0.003}\tikzmark{zinc} & 0.1606 ± 0.0015\tikzmark{code} & \third{0.3066 ± 0.0013}\tikzmark{molpcba} \\
& MPGNN+VN & 0.085 ± 0.003 (-0.18) & 0.1855 ± 0.0018 (+0.0249) & \first{0.3141 ± 0.0019} (+0.0075) \\
\bottomrule
\end{tabular}
}
}
% \end{tiny}
\end{center}

\vskip -0.1in
\end{table*}%}
% \begin{tikzpicture}[remember picture, overlay,baseline=-5ex]
%     \draw[->,rwth-red,line width=0.5pt] ($(pic cs:zinc) + (0.05,0.1)$) to[out=0, in=30] ($(pic cs:zinc) + (0.05,-0.2)$);
%     \node[anchor=west,rwth-red] (zinc) at ($(pic cs:zinc) + (0.1,-0.05)$) {-0.18};

%     \draw[->,rwth-red,line width=0.5pt] ($(pic cs:code) + (0.05,0.1)$) to[out=0, in=30] ($(pic cs:code) + (0.05,-0.2)$);
%     \node[anchor=west,rwth-red] (zinc) at ($(pic cs:code) + (0.1,-0.05)$) {-0.18};

%     \draw[->,rwth-red,line width=0.5pt] ($(pic cs:molpcba) + (0.05,0.1)$) to[out=0, in=30] ($(pic cs:molpcba) + (0.05,-0.2)$);
%     \node[anchor=west,rwth-red] (zinc) at ($(pic cs:molpcba) + (0.1,-0.05)$) {-0.18};
% \end{tikzpicture}

==> Tables/PASCAL-HP.tex <==
\begin{table}[t]
\caption{
    Hyperparameters on PascalVOC-SP.
}
\label{pascal_hp}
\begin{center}
\begin{small}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
      & GCN & GINE & GatedGCN & GPS \\
\midrule
lr              & 0.001 & 0.001 & 0.001 & 0.001 \\
dropout         & 0.0 & 0.2 & 0.2 & 0.1 \\
\#layers        & 10 & 10 & 10 & 8 \\
hidden dim.     & 200 & 145 & 95 & 68 \\
head depth      & 3 & 2 & 2 & 2 \\
PE/SE           & RWSE & none & none & LapPE \\
batch size      & 50 & 50 & 50 & 50 \\
\#epochs        & 200 & 200 & 200 & 200 \\
norm            & - & - & - & BatchNorm \\
MPNN            & - & - & - & GatedGCN \\
\#Param.        & 490k & 450k & 473k & 501k \\
\end{tabular}
}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%}


==> Tables/PCQM-HP.tex <==
\begin{table}[t]
\caption{
    Hyperparameters on PCQM-Contact.
}
\label{pcqm_hp}
\begin{center}
\begin{small}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
      & GCN & GINE & GatedGCN & GPS \\
\midrule
lr              & 0.001 & 0.001 & 0.001 & 0.001 \\
dropout         & 0.1 & 0.1 & 0.1 & 0.0 \\
\#layers        & 8 & 8 & 8 & 6 \\
hidden dim.     & 215 & 160 & 105 & 76 \\
head depth      & 1 & 1 & 1 & 1 \\
PE/SE           & LapPE & LapPE & LapPE & LapPE \\
batch size      & 500 & 500 & 500 & 500 \\
\#epochs        & 150 & 150 & 150 & 150 \\
norm            & - & - & - & LayerNorm \\
MPNN            & - & - & - & GatedGCN \\
\#Param.        & 456k & 466k & 477k & 478k \\
\end{tabular}
}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%}


==> Tables/PEPFUNC-HP.tex <==
\begin{table}[t]
\caption{
    Hyperparameters on Peptides-Func
}
\label{pepfunc_hp}
\begin{center}
\begin{small}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
      & GCN & GINE & GatedGCN & GPS \\
\midrule
lr              & 0.001 & 0.001 & 0.001 & 0.001 \\
dropout         & 0.1 & 0.1 & 0.1 & 0.1 \\
\#layers        & 6 & 8 & 10 & 6 \\
hidden dim.     & 235 & 160 & 95 & 76 \\
head depth      & 3 & 3 & 3 & 2 \\
PE/SE           & RWSE & RWSE & RWSE & LapPE \\
batch size      & 200 & 200 & 200 & 200 \\
\#epochs        & 250 & 250 & 250 & 250 \\
norm            & - & - & - & BatchNorm \\
MPNN            & - & - & - & GatedGCN \\
\#Param.        & 486k & 491k & 493k & 479k \\
\end{tabular}
}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%}


==> Tables/PEPSTRUCT-HP.tex <==
\begin{table}[t]
\caption{
    Hyperparameters on Peptides-Struct.
}
\label{pepstruct_hp}
\begin{center}
\begin{small}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
      & GCN & GINE & GatedGCN & GPS \\
\midrule
lr              & 0.001 & 0.001 & 0.001 & 0.001 \\
dropout         & 0.1 & 0.1 & 0.1 & 0.1 \\
\#layers        & 6 & 10 & 8 & 8 \\
hidden dim.     & 235 & 145 & 100 & 64 \\
head depth      & 3 & 3 & 3 & 2 \\
PE/SE           & LapPE & LapPE & LapPE & LapPE \\
batch size      & 200 & 200 & 200 & 200 \\
\#epochs        & 250 & 250 & 250 & 250 \\
norm            & - & - & - & BatchNorm \\
MPNN            & - & - & - & GatedGCN \\
\#Param.        & 488k & 492k & 445k & 452k \\
\end{tabular}
}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%}


==> Tables/PEPTIDES.tex <==

% 

% \cellcolor{blue!25} allows to color individual cells

\setlength{\tabcolsep}{3pt}
\begin{small}
\resizebox{\textwidth}{!}{
\textsc{
\begin{tabular}{l@{\hspace{4pt}}l@{\hspace{2pt}}c@{\hspace{4pt}}l@{\hspace{7pt}}c@{\hspace{4pt}}l@{\hspace{3pt}}}
\toprule
&Method     & \multicolumn{2}{c}{PEPTIDES-FUNC} & \multicolumn{2}{c}{PEPTIDES-STRUCT} \\
&           & Test AP $\uparrow$ & \!\!\!\!rel imp\!\!\!\!\!\!& Test MAE $\downarrow$ & \rlap{\!\!rel imp\!\!\!}\\
\midrule
\multirow{6}*{\rotatebox{90}{LRGB}}
&\hyperlink{cite.kipf2017semi}{GCN}                      & 0.5930 ± 0.0023 & & 0.3496 ± 0.0013 & \\
&\hyperlink{cite.Keyulu18}{GINE}                         & 0.5498 ± 0.0079 & & 0.3547 ± 0.0045 & \\
&\hyperlink{cite.bresson2017residual}{GatedGCN}          & 0.6069 ± 0.0035 & & 0.3357 ± 0.0006 & \\
&\hyperlink{cite.dwivedi2020generalization}{Transformer} & 0.6326 ± 0.0126 & & 0.2529 ± 0.0016 & \\
&\hyperlink{cite.kreuzer2021rethinking}{SAN}             & 0.6439 ± 0.0075 & & 0.2545 ± 0.0012 & \\
&\hyperlink{cite.rampavsek2022recipe}{GPS}               & 0.6535 ± 0.0041 & & 0.2500 ± 0.0005 & \\
\midrule
\multirow{4}*{\rotatebox{90}{Ours}}
&GCN                                                     & 0.6860 ± 0.0050 &\cellcolor{rwth-green!48}+16\% & \textbf{0.2460 ± 0.0007} &\cellcolor{rwth-green!90}+30\%               \\
&GINE                                                    & 0.6621 ± 0.0067 &\cellcolor{rwth-green!60}+20\% & 0.2473 ± 0.0017 &\cellcolor{rwth-green!90}+30\%                        \\
&GatedGCN                                                & 0.6765 ± 0.0047 &\cellcolor{rwth-green!33}+11\% & 0.2477 ± 0.0009 &\cellcolor{rwth-green!78}+26\%                        \\
&GPS                                                     & 0.6534 ± 0.0091 &\cellcolor{rwth-green!0}±\phantom{0}0\% & 0.2509 ± 0.0014 &\cellcolor{rwth-green!0}±\phantom{0}0\%      \\
\midrule
\multirow{6}*{\rotatebox{90}{Others}}
&\hyperlink{cite.crawl}{\textsc{CRaWl}}                                          & 0.7074 ± 0.0032 & & 0.2506 ± 0.0022 & \\
&\hyperlink{cite.pmlr-v202-gutteridge23a}{DRew}               & \textbf{0.7150 ± 0.0044} & & 0.2536 ± 0.0015 & \\
&\hyperlink{cite.shirzad2023exphormer}{Exphormer}             & 0.6527 ± 0.0043 & & 0.2481 ± 0.0007 & \\
&\hyperlink{cite.ma2023GraphInductiveBiases}{GRIT}            & 0.6988 ± 0.0082 & & \textbf{0.2460 ± 0.0012} & \\
&\hyperlink{cite.cite.pmlr-v202-he23a}{Graph ViT}             & 0.6942 ± 0.0075 & & \textbf{0.2449 ± 0.0016} & \\
&\hyperlink{cite.pmlr-v202-he23a}{G-MLPMixer}         & 0.6921 ± 0.0054 & & 0.2475 ± 0.0015 & \\
\bottomrule
\end{tabular}
}
}
\end{small}


% \begin{small}
% \resizebox{\textwidth}{!}{
% \textsc{
% \begin{tblr}{
%     colspec = {Q[c,m]Q[l,m]Q[c]Q[c]},
%     hline{1,18} = {1pt},
%     hline{2,8,12} = {0.6pt},
%     rowsep = 0pt,
%     rowsep{2} = 10pt,
%     colsep = 0.2em,
%     }
% % \toprule
% &Method     & {PEPTIDES-FUNC\\ Test AP $\uparrow$} & {PEPTIDES-STRUCT\\Test MAE $\downarrow$}  \\
% % \cline{2-3}
% \SetCell[r=6]{c} \rotatebox{90}{LRGB}&\hyperlink{cite.kipf2017semi}{GCN}                      & 0.5930 ± 0.0023 & 0.3496 ± 0.0013 \\
% &\hyperlink{cite.Keyulu18}{GINE}                         & 0.5498 ± 0.0079 & 0.3547 ± 0.0045 \\
% &\hyperlink{cite.bresson2017residual}{GatedGCN}          & 0.6069 ± 0.0035 & 0.3357 ± 0.0006 \\
% &\hyperlink{cite.dwivedi2020generalization}{Transformer} & 0.6326 ± 0.0126 & 0.2529 ± 0.0016 \\
% & \hyperlink{cite.kreuzer2021rethinking}{SAN}             & 0.6439 ± 0.0075 & 0.2545 ± 0.0012 \\
% &\hyperlink{cite.rampavsek2022recipe}{GPS}               & 0.6535 ± 0.0041 & 0.2500 ± 0.0005 \\
% % \midrule
% &GCN                                                     & 0.6860 ± 0.0050 & \textbf{0.2459 ± 0.0007} \\
% &GINE                                                    & 0.6621 ± 0.0067 & 0.2472 ± 0.0017 \\
% &GatedGCN                                                & 0.6765 ± 0.0047 & 0.2477 ± 0.0009 \\
% &GPS                                                     & 0.6533 ± 0.0091 & 0.2509 ± 0.0014 \\
% %MPNN+TL                                                 & \textbf{0.6914 ± 0.0064} & 0.2508 ± 0.0009 \\
% % \midrule
% &\textsc{CRaWl}                                          & 0.7074 ± 0.0032 & 0.2506 ± 0.0022 \\
% &\hyperlink{pmlr-v202-gutteridge23a}{DRew}               & \textbf{0.7150 ± 0.0044} & 0.2536 ± 0.0015 \\
% &\hyperlink{shirzad2023exphormer}{Exphormer}             & 0.6527 ± 0.0043 & 0.2481 ± 0.0007 \\
% &\hyperlink{ma2023GraphInductiveBiases}{GRIT}            & 0.6988 ± 0.0082 & \textbf{0.2460 ± 0.0012} \\
% &\hyperlink{cite.pmlr-v202-he23a}{Graph ViT}             & 0.6942 ± 0.0075 & \textbf{0.2449 ± 0.0016} \\
% &\hyperlink{cite.pmlr-v202-he23a}{GraphMLPMixer}         & 0.6921 ± 0.0054 & 0.2475 ± 0.0015 \\
% % \bottomrule
% \end{tblr}
% }
% }
% \end{small}

==> Tables/SP.tex <==
\setlength{\tabcolsep}{3pt}

\begin{small}
\resizebox{\textwidth}{!}{
\textsc{
\begin{tabular}{l@{\hspace{4pt}}l@{\hspace{2pt}}c@{\hspace{4pt}}l@{\hspace{7pt}}c@{\hspace{4pt}}l@{\hspace{3pt}}}
\toprule
&Method     & \multicolumn{2}{c}{PASCALVOC-SP} & \multicolumn{2}{c}{COCO-SP} \\
&           & Test F1 $\uparrow$ & \!\!\!\!rel imp\!\!\!\!\!\!& Test F1 $\uparrow$ & \rlap{\!\!rel imp\!\!\!}\\
\midrule
\multirow{6}*{\rotatebox{90}{LRGB}}&\hyperlink{cite.kipf2017semi}{GCN}                       & 0.1268 ± 0.0060\clap{\,~$^\star$} & & 0.0841 ± 0.0010\clap{\,~$^\star$} & \\
&\hyperlink{cite.Keyulu18}{GINE}                         & 0.1265 ± 0.0076\clap{\,~$^\star$} & & 0.1339 ± 0.0044\clap{\,~$^\star$} &\\
&\hyperlink{cite.bresson2017residual}{GatedGCN}          & 0.2873 ± 0.0219\clap{\,~$^\star$} & & 0.2641 ± 0.0045\clap{\,~$^\star$} &\\
&\hyperlink{cite.dwivedi2020generalization}{Transformer} & 0.2694 ± 0.0098\clap{\,~$^\star$} & & 0.2618 ± 0.0031\clap{\,~$^\star$} &\\
&\hyperlink{cite.kreuzer2021rethinking}{SAN}             & 0.3230 ± 0.0039\clap{\,~$^\star$} & & 0.2592 ± 0.0158\clap{\,~$^\star$} &\\
&\hyperlink{cite.rampavsek2022recipe}{GPS}               & 0.3748 ± 0.0109\clap{\,~$^\star$} & & 0.3412 ± 0.0044\clap{\,~$^\star$} &\\
\midrule
\multirow{4}*{\rotatebox{90}{Ours}}&GCN                  & 0.2078 ± 0.0031           & \cellcolor{rwth-green!64}+64\% & 0.1338 ± 0.0007 & \cellcolor{rwth-green!59}+59\% \\
&GINE                                                    & 0.2718 ± 0.0054           & \cellcolor{rwth-green!100}+115\% & 0.2125 ± 0.0009 & \cellcolor{rwth-green!59}+59\% \\
&GatedGCN                                                & 0.3880 ± 0.0040           & \cellcolor{rwth-green!35}+35\% & 0.2922 ± 0.0018 & \cellcolor{rwth-green!11}+11\% \\
%MPNN+TL     & 0.4241 ± 0.0030           & 0.3235 ± 0.0063 \\
&GPS                                                     & 0.4440 ± 0.0065  & \cellcolor{rwth-green!18}+18\% & \textbf{0.3884 ± 0.0055} & \cellcolor{rwth-green!13}+13\% \\
\midrule
\multirow{3}*{\rotatebox{90}{Others}}&\hyperlink{cite.crawl}{\textsc{CRaWl}}     & \textbf{0.4588 ± 0.0079} & & - & \\
&\hyperlink{cite.pmlr-v202-gutteridge23a}{DRew}               & 0.3314 ± 0.0024\clap{\,~$^\star$} & & - & \\
&\hyperlink{cite.shirzad2023exphormer}{Exphormer}             & 0.3960 ± 0.0027\clap{\,~$^\star$} & & 0.3430 ±0.0008\clap{\,~$^\star$} & \\
\bottomrule
\end{tabular}
}
}
\end{small}

==> Tables/table-slides.tex <==
\newcommand{\first}[1]{\textcolor{rwth-green}{\textbf{#1}}}
\newcommand{\second}[1]{\textcolor{rwth-blue}{\textbf{#1}}}
\newcommand{\third}[1]{\textcolor{rwth-orange}{\textbf{#1}}}

\begin{table}[t]
%\caption{
%    Performance measurements of VN-equipped models.
%    \first{First}, \second{second}, and \third{third} best values are colored.
%    % Methods marked with $^*$ did not use feature normalization on the computer vision datasets.
%    $^*$ indicates methods lacking feature normalization on the computer vision datasets.
%}
%\label{tab:lrgb_results_vn}
\begin{center}
% \begin{small}
\resizebox{\textwidth}{!}{
\textsc{
\begin{tabular}{l@{\hspace{0.7em}}lcccccc}
\toprule
&Method      & PASCALVOC-SP & COCO-SP & PEPTIDES-FUNC & PEPTIDES-STRUCT & OGB-CODE2 & OGB-MolPCBA \\
            & & Test F1 $\uparrow$ & Test F1 $\uparrow$ & Test AP $\uparrow$ & Test MAE $\downarrow$ & Test F1 $\uparrow$ & Test AP $\uparrow$ \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\small MPGNN\!}}
&\hyperlink{cite.tonshoff2023reassessingLRGB}{GCN}         & 0.2078 ± 0.0031 & 0.1338 ± 0.0007 & \first{0.6860 ± 0.0050} & \first{0.2460 ± 0.0007} & 0.1507 ± 0.0018 & 0.2483 ± 0.0037 \\
&\hyperlink{cite.tonshoff2023reassessingLRGB}{GINE} / GIN        & 0.2718 ± 0.0054 & 0.2125 ± 0.0009 & 0.6621 ± 0.0067 & \second{0.2473 ± 0.0017} & 0.1495 ± 0.0023 & 0.2703 ± 0.0023 \\
&\hyperlink{cite.tonshoff2023reassessingLRGB}{GatedGCN}    & 0.3880 ± 0.0040 & 0.2922 ± 0.0018 & 0.6765 ± 0.0047 & 0.2477 ± 0.0009 & 0.1606 ± 0.0015 & \second{0.3066 ± 0.0013} \\
% &\hyperlink{cite.cai2023connection}{MPGNN+VN ($>500\!\operatorname{k}$)} & 0.3103 ± 0.0068 & - & 0.6685 ± 0.0062 & 0.2488 ± 0.0021 & 0.1719 ± 0.0013 & 0.2848 ± 0.0026 \\
% &\hyperlink{cite.gutteridge2023drew}{DRew}                 & 0.3314 ± 0.0024 & - & \first{0.7150 ± 0.0044} & 0.2536 ± 0.0015 \\
% &\hyperlink{cite.toenshoff2023walking}{CRaWl} & \first{0.4588 ± 0.0079} & - & \second{0.7074 ± 0.0032} & 0.2506 ± 0.0022\\
\midrule
\multirow{4}{*}{\rotatebox{90}{\small GTs}}
&\hyperlink{cite.kreuzer2021rethinking}{SAN}               & 0.3230 ± 0.0039\clap{~~$^\star$} & 0.2592 ± 0.0158\clap{~~$^\star$} & 0.6439 ± 0.0075 & 0.2545 ± 0.0012 & - & 0.2765 ± 0.0042 \\
&\hyperlink{cite.rampavsek2022recipe}{GPS}                 & \second{0.4440 ± 0.0065} & \first{0.3884 ± 0.0055} & 0.6534 ± 0.0091 & 0.2509 ± 0.0014 & \second{0.1894 ± 0.0024} & 0.2907 ± 0.0028\\
& \hyperlink{cite.lgi-gt}{LGI-GT} &- & - & - & - & \first{0.1948 ± 0.0024} & \third{0.3040 ± 0.0029} \\
% &\hyperlink{cite.he2023generalization}{Graph-ViT} ($>500\!\operatorname{k}$)          & - & - & 0.6876 ± 0.0059 & \first{0.2449 ± 0.0016} & - & - \\
&\hyperlink{cite.shirzad2023exphormer}{Exphormer}          & \third{0.3975 ± 0.0037\clap{~~$^\star$}} & \second{0.3455 ± 0.0009\clap{~~$^\star$}} & 0.6527 ± 0.0043 & 0.2481 ± 0.0007 & - & - \\
% &\hyperlink{cite.ma2023graph}{GRIT} & - & - & \third{0.6988 ± 0.0082} & \third{0.2460 ± 0.0012} & - & -\\
% &\hyperlink{cite.ngo2023multiresolution}{MGT + WavePE} & - & - & 0.6817 ± 0.0064 & \second{0.2453 ± 0.0025} & - & - \\
\midrule
\multirow{2}{*}{\rotatebox{90}{\small VN}}
&GCN-VN      & 0.2950 ± 0.0058 &  0.2072 ± 0.0043  & \third{0.6732 ± 0.0066} & {0.2505 ± 0.0022} & - & - \\
&GatedGCN-VN\!\!\! & \first{0.4477 ± 0.0137} & \third{0.3244 ± 0.0025} & \second{0.6823 ± 0.0069} & \third{0.2475 ± 0.0018} & \third{0.1855 ± 0.0018}  & \first{0.3141 ± 0.0019}  \\
\bottomrule
\end{tabular}
}
}
% \end{small}
\end{center}
\vskip -0.1in
\end{table}
%}


==> Tables/vn_experiment_poster.tex <==
% \begin{table*}[t]
% \caption{
%     Performance measurements of VN-equipped models.
%     \first{First}, \second{second}, and \third{third} best values are colored.
%     % Methods marked with $^*$ did not use feature normalization on the computer vision datasets.
%     $^*$ indicates methods lacking feature normalization on the computer vision datasets.
% }
% \label{tab:lrgb_results_vn}
% \begin{center}
% % \begin{small}
\resizebox{\textwidth}{!}{
\textsc{
\begin{tabular}{l@{\hspace{0.7em}}lccccc}
\toprule
&Method      & PASCALVOC-SP & COCO-SP & PEPTIDES-FUNC & PEPTIDES-STRUCT & OGB-MolPCBA \\
            & & Test F1 $\uparrow$ & Test F1 $\uparrow$ & Test AP $\uparrow$ & Test MAE $\downarrow$ & Test AP $\uparrow$ \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\small MPGNN\!}}
&\hyperlink{cite.tonshoff2023reassessingLRGB}{GCN}         & 0.2078 ± 0.0031 & 0.1338 ± 0.0007 & \first{0.6860 ± 0.0050} & \first{0.2460 ± 0.0007} & 0.2483 ± 0.0037 \\
&\hyperlink{cite.tonshoff2023reassessingLRGB}{GINE} / GIN        & 0.2718 ± 0.0054 & 0.2125 ± 0.0009 & 0.6621 ± 0.0067 & \second{0.2473 ± 0.0017} & 0.2703 ± 0.0023 \\
&\hyperlink{cite.tonshoff2023reassessingLRGB}{GatedGCN}    & 0.3880 ± 0.0040 & 0.2922 ± 0.0018 & 0.6765 ± 0.0047 & 0.2477 ± 0.0009  & \second{0.3066 ± 0.0013} \\
% &\hyperlink{cite.cai2023connection}{MPGNN+VN ($>500\!\operatorname{k}$)} & 0.3103 ± 0.0068 & - & 0.6685 ± 0.0062 & 0.2488 ± 0.0021 & 0.1719 ± 0.0013 & 0.2848 ± 0.0026 \\
% &\hyperlink{cite.gutteridge2023drew}{DRew}                 & 0.3314 ± 0.0024 & - & \first{0.7150 ± 0.0044} & 0.2536 ± 0.0015 \\
% &\hyperlink{cite.toenshoff2023walking}{CRaWl} & \first{0.4588 ± 0.0079} & - & \second{0.7074 ± 0.0032} & 0.2506 ± 0.0022\\
\midrule
\multirow{4}{*}{\rotatebox{90}{\small GTs}}
&\hyperlink{cite.kreuzer2021rethinking}{SAN}               & 0.3230 ± 0.0039\clap{~~$^\star$} & 0.2592 ± 0.0158\clap{~~$^\star$} & 0.6439 ± 0.0075 & 0.2545 ± 0.0012 & 0.2765 ± 0.0042 \\
&\hyperlink{cite.rampavsek2022recipe}{GPS}                 & \second{0.4440 ± 0.0065} & \first{0.3884 ± 0.0055} & 0.6534 ± 0.0091 & 0.2509 ± 0.0014 & 0.2907 ± 0.0028\\
& \hyperlink{cite.lgi-gt}{LGI-GT} &- & - & - & - & \third{0.3040 ± 0.0029} \\
% &\hyperlink{cite.he2023generalization}{Graph-ViT} ($>500\!\operatorname{k}$)          & - & - & 0.6876 ± 0.0059 & \first{0.2449 ± 0.0016} & - & - \\
&\hyperlink{cite.shirzad2023exphormer}{Exphormer}          & \third{0.3975 ± 0.0037\clap{~~$^\star$}} & \second{0.3455 ± 0.0009\clap{~~$^\star$}} & 0.6527 ± 0.0043 & 0.2481 ± 0.0007 & - \\
% &\hyperlink{cite.ma2023graph}{GRIT} & - & - & \third{0.6988 ± 0.0082} & \third{0.2460 ± 0.0012} & - & -\\
% &\hyperlink{cite.ngo2023multiresolution}{MGT + WavePE} & - & - & 0.6817 ± 0.0064 & \second{0.2453 ± 0.0025} & - & - \\
\midrule
\multirow{2}{*}{\rotatebox{90}{\small VN}}
&GCN-VN      & 0.2950 ± 0.0058 &  0.2072 ± 0.0043  & \third{0.6732 ± 0.0066} & {0.2505 ± 0.0022} & - \\
&GatedGCN-VN\!\!\! & \first{0.4477 ± 0.0137} & \third{0.3244 ± 0.0025} & \second{0.6823 ± 0.0069} & \third{0.2475 ± 0.0018} & \first{0.3141 ± 0.0019}  \\
\bottomrule
\end{tabular}
}
}
% {
% \footnotesize
~\smallskip
% \singlespacing
% \fontsize{9}{8}\selectfont
% \linespread{0.7}

Best results shown as: \first{First}, \second{Second}, \third{Third}. MPGNN+VN architectures compete well with GTs, indicating that none is trivially better. New SOTA on molPCBA using GatedGCN+VN.
% }
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}
% %}

